Turaev Hyperbolicity of Classical and Virtual Knots

By work of W. Thurston, knots and links in the 3-sphere are known to either be torus links, or to contain an essential torus in their complement, or to be hyperbolic, in which case a unique hyperbolic volume can be calculated for their complement. We employ a construction of Turaev to associate a family of hyperbolic 3-manifolds of finite volume to any classical or virtual link, even if non-hyperbolic. These are in turn used to define the Turaev volume of a link, which is the minimal volume among all the hyperbolic 3-manifolds associated via this Turaev construction. In the case of a classical link, we can also define the classical Turaev volume, which is the minimal volume among all the hyperbolic 3-manifolds associated via this Turaev construction for the classical projections only. We then investigate these new invariants.

==> abstract.tex <==
By work of W. Thurston, knots and links in the 3-sphere are known to either be torus links, or to contain an essential torus in their complement, or to be hyperbolic, in which case a unique hyperbolic volume can be calculated for their complement. We employ a construction of Turaev to associate a family of hyperbolic 3-manifolds of finite volume to any classical or virtual link, even if non-hyperbolic. These are in turn used to define the \emph{Turaev volume} of a link, which is the minimal volume among all the hyperbolic 3-manifolds associated via this Turaev construction. In the case of a classical link, we can also define the \emph{classical Turaev volume}, which is the minimal volume among all the hyperbolic 3-manifolds associated via this Turaev construction for the classical projections only.   We then investigate these new invariants.

==> holes.tex <==
% For a classical link projection $D_L$ of a link $L$ with Gauss code $G$, we provide an algorithm that takes $G$ as an input, and outputs the Gauss code for a link $L_s$ such that surgery on $L_s$ gives the complement of $L$'s lifting in it's turaev surface. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/turaev_holes.png}
%     \caption{An unknot projection, its $A$ state circles, its $B$ state circles, and its genus $3$ turaev surface viewed from above, revealing the holes.}
%     \label{fig:turaev_holes}
% \end{figure}

% We start by finding the holes. Diagrammatically, the holes will correspond to some complementary regions of the knot projection that do not get capped off in the turaev construction. This process can be seen in Figure~\ref{fig:turaev_holes}. 

==> homelesslemmas.tex <==
% \begin{lemma}
%     A turaev surface has no cancellation curves.
% \end{lemma}
% \begin{proof}
%     {\color{red}Proof sketch: }The orientable case follows from fully alternating. The unorientable case follows from taking the double cover (orientable double cover is fully alternating, cancellation curve in nonorientable surface would lift to cancellation curve upstairs, write this up nicely) (the projection on the orientable double cover is the same thing you get by walking along the surface of the twisted i bundle over your non orientable turaev surface, which is by definition of turaev surface alternating)
% \end{proof}



==> hyperbolicity.tex <==

% \begin{definition}
%     Given a diagram $D$ of a virtual link, define the Turaev surface-link pair of the diagram, $\big(S_T(D), L_T(D)\big)$, to be the link which lives on the Turaev surface corresponding to the diagram $D$.
% \end{definition}

% In \cite{small2017}, the authors defined \emph{fully alternating} links in a surface cross $I$. 

% \begin{definition}
%     Let $(S,L)$ be a surface link pair where $S$ is not the sphere or projective plane. We call $(S,L)$ \emph{fully alternating} if the link $L$ is alternating on the surface and $S \smallsetminus L$ is a disjoint union of disks. 
%     A virtual link is \emph{fully alternating} if it admits a representation which is fully alternating.
% \end{definition}

% We define a cancellation curve for a link {\color{red}embedded} in $S\times I$ as follows
% \begin{definition}
% {\color{red}cancellation curve}
% \end{definition}

% The authors of \cite{small2017} showed that fully alternating links on a thickened surface have no cancellation curves, meaning they are minimal genus. The is because a cancellation curve is by definition a topologically nontrivial curve in the link complement, of which there are none in the fully alternating case. Furthermore, they provved the following.

% \begin{theorem}[\cite{small2017}]
% The complement in $S\times I$ of a prime, fully alternating link admits a finite-volume hyperbolic metric such that the boundary of $S \times I$ is totally geodesic.
% \end{theorem} 



\kabir{define and use tg-hyperbolic}

\noindent In \cite{small2017}, the authors also provided a necessary and sufficient condition for determining primeness in fully alternating surface-link pairs. They showed that a knot is prime if and only if there is a disk on the surface such that the boundary of the disk is transverse to the knot, intersects the knot twice, and such that the disk contains a nontrivial tangle.
\\\\
\noindent Since any Turaev surface-link pair is by construction fully alternating, we can assign a hyperbolic volume to any knot projection that lifts to a prime knot on its Turaev surface. In Sections~\ref{turaevprimeness} and Section~\ref{turaevvolume}, we will show that every knot has some projection whose Turaev surface admits a hyperbolic volume, and, in fact, infinitely many projections with such a volume. 

% \begin{lemma}
% A surface-link pair $(S,L)$ lifts to a prime Turaev surface-link if and only if there does not exist a disk in $S$ whose boundary intersects the link transversally in two points such that the interior of the disk contains a nontrivial alternating tangle. Equivalently, the Gauss code associated to the surface-link pair does not contains a subcode of a nontrivial classical knot. \kate{define subcode maybe?}
% \end{lemma}
% \kabir{Lemma is false}

% \begin{proof}
% If $(S,L)$ lifts to a composite Turaev surface-link pair, then there exists a disk precisely of the sort described in the lemma's statement in the Turaev surface-link pair. But then {\color{red} but then what, numbnuts?}
% \end{proof}


\noindent We now generalize the above computations. The first generalization is as follows. Let $w$ denote some word in the the letters $c,v$ and denote by $\swift{P}_n^w$ the alternating link with $|w|$ layers, each letter of $w$ corresponding to an either all classical or all virtual layer (with $n$ all classical or all virtual crossings respectively).
\\\\
First we note that $\swift{P}_n^w$ has more than one component if and only if $|w|$ divides $n$, in which case it has $n/ |w|$ components. We want to discard the cases where $\swift{P}_n^w$ is splittable. This happens if and only if $\swift{P}_n^w$ has more than one component, one of which has all of its classical crossings with itself. Following the path of this component $\swift{C}$ across the layers of $\swift{P}_n^w$, we deduce that the first and last layers of some such $\swift{P}_n^w$ must be virtual (so $w$ must start and end with a $v$). Moreover, $\swift{C}$ can only have classical crossings with itself, so this forces every letter of $w$, except precisely those whose positions in $w$ multiples of $n/|w|$, to be $v$ (the rest being $c$). In summary, we have:
\begin{proposition}
$\swift{P}_n^w$ has more than one component if and only if $|w|$ divides $n$, in which case $\swift{P}_n^w$ is splittable if and only if every letter of $w$, except precisely those whose positions in $w$ multiples of $n/|w|$, to be $v$, the rest being $c$.
\end{proposition}
\noindent We now show that any non-splittable $\swift{P}_n^w$ is hyperbolic. 
%First some lemmas: \kabir{Let's take this stuff out. Instead, let's prove hyperbolicity via the gauss code method, in the Turaev paper.}
%\begin{lemma}
    %Let $w$ denote a word in $\{c,v\}$ ending in $c$. Form the word $w'$ from $w$ by concatenating the letter $c$. Then provided both $\swift{P}_n^w, \swift{P}_n^{w'}$ are non-splittable, we have $$g(\swift{P}_n^{w'}) = g(\swift{P}_n^w).$$
%\end{lemma}
%\begin{proof}
%If without loss of generality the $B$ state of $\swift{P}_n^w$ consists of a single circle bordering on the outside, then the new $B$ state will consist of $n$ circles bordering inside the regions between the added layer and previous outer layer, while the circle that used to border the outer layer is removed. In this case the new $A$ state will consist of all the circles in the previous $A$ state, and in addition, a single circle bordering outside the added layer. In summary, the number of circles in the $A$ and $B$ states collectively rises by $n$, the number of classical crossings added. This gives the result.
%\end{proof}
%\begin{lemma}
    %Let $w$ denote a word in in $\{c,v\}$ ending in $c$. Form the word $w'$ from $w$ by concatenating the letter $v$.Then provided both $\swift{P}_n^w, \swift{P}_n^{w'}$ are non-splittable, we have $$g(\swift{P}_n^{w'}) = g(\swift{P}_n^w) - \left(\frac{n - \gcd(n,2)}{2}\right).$$
%\end{lemma}
%\begin{proof}
%If without loss of generality the $B$ state of $\swift{P}_n^w$ consists of a single circle bordering on the outside, then the new $B$ state will consist of $\gcd(n,2)$ circles bordering the outside. The $A$ state of $\swift{P}_n^w$ then consists of $n$ outer circles, one for each arc in the outer region. Adding a virtual layer then eliminates these circles and adds a single circle which meets each arc in the new outer layer. In sum, we have:
%\begin{align*}
   % g(\swift{P}_n^{w'}) = g(\swift{P}_n^{w}) + \left(\frac{\gcd(n,2) - 1 - n+ 1}{2}\right) = g(\swift{P}_n^w) - \left(\frac{n - \gcd(n,2)}{2}\right).
%\end{align*}
%\end{proof}
%\begin{lemma}
%Let $w$ denote a word in $\{c,v\}$ ending in $v$. Form the word $w'$ from $w$ by concatenating the letter $c$. Then provided both $\swift{P}_n^w, \swift{P}_n^{w'}$ are non-splittable, we have $$g(\swift{P}_n^{w'}) = g(\swift{P}_n^w) + \left(\frac{n - \gcd(n,2)}{2}\right).$$ ({\color{red}Actually idk about this})
%\end{lemma}
%\begin{proof}
%There are two w
%\end{proof}
\kate{clean up section in terms of looking at primeness}
\kabir{We should type up the gauss code proof of Polygonal knots are prime}


==> style.tex <==
\usepackage[utf8]{inputenc}
\usepackage[margin=1.3in]{geometry}
%\usepackage{color}
\usepackage{amssymb,amsmath,amsthm}
\usepackage{graphicx}
\usepackage[margin=1.5cm]{caption}
\usepackage{subcaption} %for subfigures
\usepackage{mathtools}
\usepackage{gensymb} %for \circ for \deg

\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{positioning} % for extra poositioning for chords on circles
\usetikzlibrary{through} %alternative fancy circle stuff

\usepackage{textcase}
\usepackage{microtype}

% pseudocode formatting
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\def\BState{\State\hskip-\ALG@thistlm}


% TODO NOTES: \usepackage[pdftex,dvipsnames]{xcolor}  % Coloured text etc.
%\usepackage[table,xcdraw,svgnames]{xcolor} 
\PassOptionsToPackage{svgnames}{xcolor} % svgnames gives more color options for hyperlinks
\PassOptionsToPackage{table}{xcolor} 
\PassOptionsToPackage{xcdraw}{xcolor} 


% wrapping text around figures
\usepackage{wrapfig}

% for add margin for indented blocks of text
\usepackage{scrextend}


\usepackage[titletoc,title]{appendix} % title attribute adds "Appendix A" b4 appendix title, titletoc does it in the table of conents


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SECTION HEADERS STYLING
\usepackage{titlesec}
%%%%%%%%%%%%%%%%%%%%%%%% first option %%%%%%%%%%%%%%%%%%%%%%%%
%\titleformat{\section}[block]{\Large\bfseries\centering}
%            {\thesection.\quad}{-0.6em}{}
%%%%%%%%%%%%%%%% second option: smallcaps %%%%%%%%%%%%%%%%%%%%
\titleformat{\section}[block]{\Large\scshape\centering}
            {\thesection.\quad}{-0.6em}{}
\titleformat{\subsection}{\large\centering\scshape}
            {\thesubsection.\quad}{-0.6em}{}
%%%%%%%%%%%%%%%%%%% title & name fonts %%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\TitleFont}{%
    \usefont{\encodingdefault}{ptm}{b}{sc}%
    \fontsize{14}{18}%
    \selectfont}
\newcommand*{\NameFont}{%
    \usefont{\encodingdefault}{ptm}{m}{sc}%
    \fontsize{12}{14}
    \selectfont}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BIBLIOGRAPHY FORMATTING
\usepackage[numbers,square,comma,sort&compress]{natbib}
\usepackage{ulem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINKS FORMATTING
\usepackage[colorlinks]{hyperref}
\AtBeginDocument{%
  \hypersetup{
    citecolor=green,
    linkcolor=blue,   
    urlcolor=magenta}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% USEFUL DEFINITIONS
% if loop for environment definitions
\makeatletter
\def\ifenv#1{
   \def\@tempa{#1}%
   \ifx\@tempa\@currenvir
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
   \fi
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GENERAL THEOREM STYLING
% \newtheoremstyle{mystyle}{}{}{\itshape}{}{\scshape}{.}{.5em}{}
% \theoremstyle{mystyle}
\theoremstyle{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREM ENVIROMENTS
\newtheorem{definition}{Definition}
\numberwithin{definition}{section}
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\newtheorem{fact}{Fact}
\numberwithin{fact}{section}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}

% the [theorem] tag above puts thms and lemmas in the same 
% numbering scale
% \numberwithin{lemma}{section}
\newtheorem{corollary}{Corollary}
\numberwithin{corollary}{theorem}
\newtheorem{proposition}{Proposition}
\numberwithin{proposition}{section}
\newtheorem{conjecture}{Conjecture}
\numberwithin{conjecture}{section}
\newtheorem*{remark}{Remark}
\newtheorem{question}{Question}
\numberwithin{question}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH MODE SHORTCUTS
\newcommand{\homeo}{\mbox{Hom}}
\newcommand{\thomeo}{\textup{Hom}}
\newcommand{\mcg}{\mbox{Mod}}
\newcommand{\tmcg}{\textup{Mod}}
\newcommand{\inv}{^{-1}}
\newcommand{\com}[2]{\lbrack #1, #2\rbrack} % commutator
\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\renewcommand{\deg}{^{\circ}}
\newcommand{\twotorus}{\mathbb{T}^2\#\mathbb{T}^2}

% FIX EMPH
\renewcommand{\emph}[1]{\textit{#1}}

\newcommand{\vol}{\text{vol}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Or's Command
\renewcommand{\qedsymbol}{$\blacksquare$}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\tvs}{\pitchfork}

\newcommand{\grad}{\vec{\nabla}}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\im}{\mathrm{im}}

\newcommand{\Log}{\mathrm{Log}}
\newcommand{\F}{\mathscr{F}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\DD}{\partial}
\newcommand{\dd}{\mathrm{d}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%1

%Notes

\newcommand{\nota}[1]
{\-\marginpar[\raggedleft\tiny \textcolor{colore}{#1}]{\raggedright\tiny \textcolor{colore}{#1}}}

\newcommand{\notanat}[1]
{\-\marginpar[\raggedleft\tiny \textcolor{coloregen}{#1 G}]{\raggedright\tiny \textcolor{coloregen}{#1 G}}}

\newcommand{\notakevin}[1]
{\-\marginpar[\raggedleft\tiny \textcolor{coloregen}{#1 G}]{\raggedright\tiny \textcolor{coloregen}{#1 K}}}

\newcommand{\notanick}[1]
{\-\marginpar[\raggedleft\tiny \textcolor{coloresimo}{#1 S}]{\raggedright\tiny \textcolor{coloresimo}{#1 S}}}


%TODO NOTES
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
% 
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\nat}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\oreisenberg}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\yi}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\zhen}[2][1=]{\todo[linecolor=purple,backgroundcolor=purple!25,bordercolor=purple,#1]{#2}}
\newcommandx{\jonah}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\kabir}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\kate}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}
\newcommandx{\colin}[2][1=]{\todo[linecolor=gray,backgroundcolor=gray!25,bordercolor=gray,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
%


%MY SHORTCUTE
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\Z}{\mathbb{Z}}
% \newcommand{\Q}{\mathbb{Q}}

\usepackage{blkarray} %blockarray- matrices with labels
%\usepackage{caption} %adjust figure caption widths

\usepackage[]{caption}

\usepackage{floatrow}

==> turaevgenus.tex <==
\kate{change to a remark}

Recall that the Turaev surface of a link diagram $D_L$ for a link $L$ is a cobordism between the all-A and all-B smoothings of $D_L$, where the boundary components are then capped off with disks. As such, the genus of the Turaev surface for $D_L$ is 
$$g = \frac{c(D_L) - |S_A(D_L)|- |S_B(D_L)| + 2}{2} $$
where $c(D_L)$ denotes number of crossings in $D_L$, and $|S_A(D_L)|$ and $|S_B(D_L)|$ denote the number of circles in the $A$ and $B$ smoothings of $D_L$, respectively. It is possible to tell, from the Gauss code of $D_L$, what $|S_A(D_L)|, |S_B(D_L)|$ are, and we present an algorithm to do so. 

To compute the amount of circles in the $A$ smoothing of a diagram with gauss code $G$, we realize a ``walk'' on the Gauss code that corresponds to ``walking'' along the state circle. We say that we are walking ``forward'' if we are walking in the same direction as the orientation of the link diagram, and ``backward'' otherwise. 
In {\color{red}figure} we can see that if we are walking along a circle in the $A$ smoothing and we meet a positive writhe crossing while walking forward, we change strands and continue to walk forward. On the other hand if we meet a negative write crossing, in order to continue walking along the same state circle we must change strands and then walk backward. The process is captured in Algorithm~\ref{algorithm:find_loop}.


{\color{red}explain it?}

% \begin{algorithm}
% \caption{Computing a loop in the $A$-smoothing}\label{algorithm:find_loop}
% \begin{algorithmic}[1]
% \State $\textit{current crossing}\gets \text{crossing at }\textit{starting position}$
% \While{\textbf{not} (\textit{current position = starting position} and \textit{direction = forward})}:
%     \State $\textit{current position} \gets\text{next occurrence of }\textit{current crossing}$\Comment{Change strands}
%     \If{writhe of \textit{current crossing} is negative}
%         \State$\textit{direction}\gets\text{opposite direction}$\Comment{Change between forward/backward}
%     \EndIf
%     \State $\textit{current position}\gets\textit{current position + direction}$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
We can compute state circles starting at each position in the Gauss code, and then eliminate redundancies by eliminating state circles that are cyclic permutations or reversed cyclic permutations of each other. 

The algorithm for the $B$ smoothing is almost the same, except we change direction on positive write crossings instead of negative writhe crossings, as seen in {\color{red}figure}.

==> turaevprimeness.tex <==
{\color{red}Note that throughout we work with \emph{reduced} link diagrams, meaning no obvious RI simplifications. }

{\color{red} we kill this for the time being}
\begin{definition}
    We say that a diagram $D_L$ for a link $L$ is \emph{Turaev prime} if it lifts to a prime link on its Turaev surface. Otherwise, we say that it is \emph{Turaev composite}.
\end{definition}

\begin{lemma}
    \label{lemma:turaevprime}
    A diagram $D_L$ is Turaev composite if and only if the corresponding Gauss code $G$ has a genus $0$ alternating sub-Gauss code. \nat{define what we mean by genus of a Gauss code and by sub-gauss code}
\end{lemma}\nat{THIS IS WRONG, UPDATE IT}

\begin{proof}
    Assume $G$ has a genus $0$ alternating sub-Gauss code $G'$. Since the sub-Gauss code is alternating, it will lift to itself in the Turaev surface of $D_L$. Since it is genus $0$, there exists a disk on the Turaev surface bounding a classical $1$ tangle (ehat's a 1-tangle?) with Gauss code $G'$. Therefore by {\color{red}prime iff obviously prime} the link in the /Turaev surface is composite. 
    The converse is straightforward. 
\end{proof}

Lemma~\ref{lemma:turaevprime} says that a virtual knot diagram is Turaev prime if and only if it is not a composition of a nontrivial classical alternating knot diagram with some other (possibly virtual) nontrivial diagram.\nat{THIS IS FALSE NOW}
